Nucleon axial charge from quenched lattice QCD with domain wall fermions

We present a quenched lattice calculation of the nucleon isovector vector and axial-vector charges gV and gA. The chiral symmetry of domain wall fermions makes the calculation of the nucleon axial charge particularly easy since the Ward-Takahashi identity requires the vector and axial-vector currents to have the same renormalization, up to lattice spacing errors of order O(a^2). The DBW2 gauge action provides enhancement of the good chiral symmetry properties of domain wall fermions at larger lattice spacing than the conventional Wilson gauge action. Taking advantage of these methods and performing a high statistics simulation, we find a significant finite volume effect between the nucleon axial charges calculated on lattices with (1.2 fm)^3 and (2.4 fm)^3 volumes (with lattice spacing, a, of about 0.15 fm). On the large volume we find gA = 1.212 +/- 0.027(statistical error) +/- 0.024(normalization error). The quoted systematic error is the dominant (known) one, corresponding to current renormalization. We discuss other possible remaining sources of error. This theoretical first principles calculation, which does not yet include isospin breaking effects, yields a value of gA only a little bit below the experimental one, 1.2670 +/- 0.0030.

==> text_sections/outline/outline_I.tex <==
%
% Intro:Outline
%

\ifnum\theOutline=1
\noindent \framebox{Begin \ outline \hspace{5.0in} }
\begin{enumerate}
%% 1
\item Four form factors appear in neutron \(\beta\) decay,
\begin{itemize}
\item the vector and induced tensor from the vector current,
\[
\langle p| V^+_\mu(x) | n \rangle
= i\bar{u}_p [\gamma_\mu g_{_V}(q^2)
             +q_\lambda \sigma_{\lambda\mu} g_{_M}(q^2) ] u_n e^{-iqx},
\]
\item and the axial and induced pseudo-scalar from the axial current,
\[
\langle p| A^+_\mu(x) | n \rangle
= i\bar{u}_p \gamma_5
             [\gamma_\mu g_{_A}(q^2)
             +q_\mu g_{_P}(q^2) ] u_n e^{-iqx}.
\]
\end{itemize}
where \(q=p_n-p_p\) is the momentum transfer.
\item In the limit of \(q^2\rightarrow 0\), the vector and axial form factors survive.  Their values are \footnote{The Particle Data Group.}:
\begin{itemize}
\item \(g_{_V} = G_F \cos \theta_C\) (\(G_F\) is the Fermi constant and \(\theta_C\) is the Cabibbo mixing angle)
\item and \(g_{_A} = g_{_V} \times 1.2670(30)\).
\end{itemize}

%% 2
\item While historically

\begin{itemize}
\item NR quark model gives \(5/3\), no size dependence,
\item MIT bag model gives 1.07 (1.09?), no size dependence?
\item connection to polarized structure function \(g_1(x)\) through the Bjorken sum rule.
\end{itemize}

%% 3
\item Theoretically \(g_{_A}\) is one of the simplest of nucleon
electroweak matrix elements:
\begin{itemize}
    \item the lowest moment
    \item zero momentum transfer
    \item no disconnected contribution (the iso-symmetric case)
\end{itemize}
%% 4
\item Failure in reproducing \(g_{_A}\) in lattice QCD
\begin{itemize}

\item lattice calculations with Wilson or clover fermions typically underestimates by up to 25 \%,

\item possible systematic errors
\begin{itemize}

\item quenching: \((g_A)^{\rm Full}< (g_A)^{\rm Quench}\) (\(\sim 5\)-\(10\% \searrow\))
\item finite lattice spacing: \((g_A)_{\rm at\;a\rightarrow 0} > (g_A)_{\rm at\;a\sim 0.1 fm}\) (\(\sim 5\%\nearrow\))
\item determination of $Z_{_A}$: \(Z_{_A}^{NP}<Z_{_A}^{P}\) (\(\sim 15\)-\(20\% \searrow\))
\item exact axial vector
\item finite volume: no estimation so far
\end{itemize}
\end{itemize}

%% 5
\item \(g_{_A}/g_{_V} \neq 1\) is strongly related to the partially
conserved axial current.
\begin{itemize}
\item Goldberger-Treiman relation (the axial WT identity)
\end{itemize}
%% 6
\item Domain wall fermions (DWF) preserves almost exact chiral symmetry on the
lattice:
\begin{itemize}
\item by introducing a fictitious fifth dimension
in which the symmetry violation is exponentially suppressed.
\item Success in: chiral symmetry and ground-state mass
spectrum~\cite{Blum:2000kn},
Kaon matrix elements~\cite{Blum:2001xb},
\(N^*\) mass~\cite{Sasaki:2001nf}, ...

\item remarkable property such as \(Z_{_A}=Z_{_V}\)
\begin{itemize}
\item \((g_{_A}/g_{_V})^{\rm lattice}\) directly yields the renormalized value of \(g_{_A}\)
\item \(Z_{_A} \neq Z_{_V}\) and other renormalization complications for Wilson and clover fermions
\end{itemize}
\end{itemize}

%% 7
\item First DWF calculation of \(g_{_A}\)
\begin{itemize}
\item fairly strong dependence on quark mass
\item chiral extrapolation yields the quite low value of \(g_{_A}\) at \(m_f=0\)
\item simulation in typical spatial size \(L\sim 1.5 {\rm fm}\): not large enough 
\end{itemize}
%% 8
\item RG improved gauge action, DBW2 (``doubly blocked Wilson 2'') action
\begin{itemize}

\item by adding rectangular (\(2 \times 1\)) Wilson loops to the action.

\item improves approach to the continuum
\begin{itemize}
\item good scaling behaviors 
\end{itemize}

\item keep good chiral properties of DWF 
\begin{itemize}

\item the ``residual mass,'' which controls low energy
chiral behavior, is driven to \(am_{\rm res} < O(10^{-4}) \) or \(\ll {\rm MeV}\).
\end{itemize}
\item simulation can be employed on coarse lattice, but in large physical volume
\end{itemize}

%%%%%

\end{enumerate}
\noindent \framebox{End \ outline \hspace{5.0in} }
\vspace{0.25in}
\fi


==> text_sections/outline/outline_II.tex <==
\ifnum\theOutline=1
\noindent \framebox{Begin \ outline \hspace{5.0in} }
\begin{enumerate}
\item Our formulation follows the standard one:
\item Form factor definition: what to do with \(G_F\) and \(\cos \theta_c\)?
\item Basic properties of the vector and axial currents: CVC and PCAC.
\begin{itemize}
\item That \(g_{_V}\) = 1 is assured within CVC: 
\item \( j_{\mu}^{em}=\frac{2}{3}V_{\mu}^{u}-\frac{1}{3}V_{\mu}^{d}+\ldots\) 
\item \( \lim_{q^2 \rightarrow 0} \langle n| j_{\mu}^{em}|n \rangle =
\langle\langle n| j_{\mu}^{em}|n \rangle\rangle=
0 \) for neutron.
\item it turns out that
\( \langle\langle p| V_{\mu}^{u}|p \rangle\rangle =2\times\langle\langle p| V_{\mu}^{d}|p \rangle\rangle\)
because of iso-symmetry.
\item consequently, 
\(\langle\langle p| j_{\mu}^{em}|p \rangle\rangle=\langle\langle p| V_{\mu}^{d}|p \rangle\rangle
=\langle\langle p| V_{\mu}^{u}-V_{\mu}^{d}|p \rangle\rangle\)
\end{itemize}
Discuss the breakings too.
\item On the lattice, in general, we calculate the relevant matrix elements of
these currents
\begin{itemize}
\item with a lattice cutoff, \(a^{-1}\) \(\sim\) 1-2 GeV,
\item and extrapolate to the continuum, \( a \rightarrow 0\),
\end{itemize}
introducing lattice renormalization: \(g_{_V, _A}^{\rm ren} = Z_{_V,
_A} g_{_V, _A}^{\rm lattice}\).

\item Also, unwanted lattice artefact may result in unphysical mixing of
chirally distinct operators.
\item \(g_{_A}\) is also described as \(\Delta u - \Delta d\): Kostas Originos talk.
\begin{itemize}
\item \( \langle p| A_{\mu}^{+}|n \rangle = \langle p| A_{\mu}^{u}-A_{\mu}^{d}|p \rangle \)
where \( A_{\mu}^{u}={\bar u}\gamma_{\mu}\gamma_{5}u\) and 
\( A_{\mu}^{d}={\bar d}\gamma_{\mu}\gamma_{5}d\) 
\end{itemize}
\item Wall source.
\item Sequential source.
\item Wilson action.
\item DBW2 improved action.
\end{enumerate}
\noindent \framebox{End \ outline \hspace{5.0in} }
\vspace{0.25in}
\fi


==> text_sections/outline/outline_IIa.tex <==
\ifnum\theOutline=1
\noindent \framebox{Begin \ outline \hspace{5.0in} }
\begin{enumerate}
% 1
\item Interpolating operator for proton ; \( {\cal N}= \epsilon_{abc} [u_a^T C \gamma_5d_b]u_c\).
% 2
\item Time-slice correlation functions (the rest frame, the zero-momentum):\\
\(
\langle {\cal N}(t){\bar {\cal N}}(0) \rangle_{\alpha \beta}
=\sum_{\vec x} \langle T\{ {\cal N}({\vec x}, t){\bar {\cal N}}({\vec 0},0)  \}\rangle_{\alpha \beta}
\)
\\
\(
\langle {\cal N}(t){\cal O}(t'){\bar {\cal N}}(0) \rangle_{\alpha \beta}
=\sum_{\vec x}\sum_{{\vec x}'}  
\langle T\{ {\cal N}({\vec x}, t){\cal O}({\vec x}', t'){\bar {\cal N}}({\vec 0},0)  \}\rangle_{\alpha \beta}
\)
% 3
\item Two-point function:\\
\(\displaystyle
G_{_N}(t) = \frac{1}{4}{\rm Tr}\{ P_{+}  \langle {\cal N}(t){\bar {\cal N}}(0) \rangle\},
\)
with the (particle and parity) projection operator \(P_{+}=(1+\gamma_4)/2\).

% 4
\item Three-point functions,
\begin{itemize}
\item vector:
\(\displaystyle
G_{_V}^{u,d}(t,t') = \frac{1}{4}{\rm Tr} \{P_{+}
\langle  {\cal N}(t){V_{4}^{u,d}}(t'){\bar {\cal N}}(0) \rangle \},
\)
\item axial:
\(\displaystyle
G_{_A}^{u,d}(t,t') = \frac{1}{4} {\rm Tr} \{
P_{+}\gamma_i\gamma_5 
\langle  {\cal N}(t){A_{i}^{u,d}}(t'){\bar {\cal N}}(0) \rangle \},
\) (\(i=1,2,3\))
\end{itemize}
with fixed \(t'=t_{\rm source}-t_{\rm sink}\) and \(t < t'\).

% 5
\item From the lattice estimate
\[
g_{_\Gamma}^{\rm lattice}
= \frac{G_{_\Gamma}^u(t,t')-G_{_\Gamma}^d(t,t')}{G_{_N}(t)},
\]
with \(\Gamma = V\) or \(A\), the continuum value
\[
g_{_\Gamma} = Z_{_\Gamma} g_{_\Gamma}^{\rm lattice},
\]
is obtained.

% 6
\item Non-perturbative renormalizations, defined by
\[
[\bar{u} \Gamma d]_{\rm ren} = Z_{_\Gamma} [\bar{u}\Gamma d]_0,
\]
satisfies \(Z_{_A} = Z_{_V}\) well, so that
\[
\left(\frac{g_{_A}}{g_{_V}}\right)^{\rm ren} =
\left(
\frac{G_{_A}^u(t,t')-G_{_A}^d(t,t')}{G_{_V}^u(t,t')-G_{_V}^d(t,t')}
\right)^{\rm lattice}.
\]
\end{enumerate}
\noindent \framebox{End \ outline \hspace{5.0in} }
\vspace{0.25in}
\fi

